Fault Localization in Web Applications via Model Finding

We describe a generic technique for fault localization independent from the nature of the object or the specification language used to declare its expected properties. This technique is based on the concept of "repair", a minimal set of transformations which, when applied to the original object, restores its satisfiability with respect to the specification. We show how this technique can be applied with various specification languages, including propositional and finite first-order logic. In particular, we focus on its use in the detection of layout faults in web applications.

==> eptcsdata.tex <==
\providecommand{\firstpage}{55}
\providecommand{\publicationstatus}{G. G\"ossler and O. Sokolsky (Eds.): 1st Workshop on Causal Reasoning for \\ Embedded and safety-critical Systems Technologies (CREST'16)\\
EPTCS 224, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.224.6}{10.4204/EPTCS.224.6}}
\pdfoutput=1

